Gepner-like boundary states on $T^4$

We present exact expressions for elementary boundary states which describe D-branes preserving 16 or fewer supercharges in type II superstring compactified on certain self-dual 4-tori. While being manifestly superconformal, our boundary states are not a priori required to satisfy the usual free-field gluing conditions along the internal directions of the 4-tori. Our calculations proceed along the lines of Gepner's construction by recasting the $\mathcal{N}=(2,2)$ worldsheet sigma model on the 4-tori in terms of $\mathcal{N}=2$ minimal models. Imposing general permutation gluing conditions on the $\mathcal{N}=(2,2)$ generators is shown to yield various stable and unstable D-branes, where the stable ones include the known 1/2-BPS and 1/4-BPS bound states of D$p$-branes, as well as new non-BPS D-branes, which do not carry RR charges.

==> nonBPSpot.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  % Encoding inside the plot.  In the header of your document, this encoding
  % should to defined, e.g., by using
  % \usepackage[cp1250,<other encodings>]{inputenc}
  \inputencoding{cp1250}%
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(8502.00,5668.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,704){\makebox(0,0)[r]{\strut{}$-1.0$}}%
      \put(946,1178){\makebox(0,0)[r]{\strut{}$-0.9$}}%
      \put(946,1653){\makebox(0,0)[r]{\strut{}$-0.8$}}%
      \put(946,2127){\makebox(0,0)[r]{\strut{}$-0.7$}}%
      \put(946,2601){\makebox(0,0)[r]{\strut{}$-0.6$}}%
      \put(946,3075){\makebox(0,0)[r]{\strut{}$-0.5$}}%
      \put(946,3550){\makebox(0,0)[r]{\strut{}$-0.4$}}%
      \put(946,4024){\makebox(0,0)[r]{\strut{}$-0.3$}}%
      \put(946,4498){\makebox(0,0)[r]{\strut{}$-0.2$}}%
      \put(946,4973){\makebox(0,0)[r]{\strut{}$-0.1$}}%
      \put(946,5447){\makebox(0,0)[r]{\strut{}$0.0$}}%
      \put(1078,484){\makebox(0,0){\strut{}$0$}}%
      \put(1850,484){\makebox(0,0){\strut{}$1$}}%
      \put(2622,484){\makebox(0,0){\strut{}$2$}}%
      \put(3395,484){\makebox(0,0){\strut{}$3$}}%
      \put(4167,484){\makebox(0,0){\strut{}$4$}}%
      \put(4939,484){\makebox(0,0){\strut{}$5$}}%
      \put(5711,484){\makebox(0,0){\strut{}$6$}}%
      \put(6483,484){\makebox(0,0){\strut{}$7$}}%
      \put(7256,484){\makebox(0,0){\strut{}$8$}}%
      \put(8028,484){\makebox(0,0){\strut{}$9$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,3075){\rotatebox{-270}{\makebox(0,0){\strut{}$V(r;d_\bot)$}}}%
      \put(4591,154){\makebox(0,0){\strut{}$r$}}%
      \csname LTb\endcsname%%
      \put(7118,1317){\makebox(0,0)[r]{\strut{}$d_\bot = 3$}}%
      \csname LTb\endcsname%%
      \put(7118,1097){\makebox(0,0)[r]{\strut{}$d_\bot = 4$}}%
      \csname LTb\endcsname%%
      \put(7118,877){\makebox(0,0)[r]{\strut{}$d_\bot = 5$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{nonBPSpot}}%
    \gplfronttext
  \end{picture}%
\endgroup

